Automated Curvy Waveguide Routing for Large-Scale Photonic Integrated Circuits

As photonic integrated circuit (PIC) designs advance and grow in complexity, largely driven by innovations in photonic computing and interconnects, traditional manual physical design processes have become increasingly cumbersome. Available PIC layout automation tools are mostly schematic-driven, which has not alleviated the burden of manual waveguide planning and layout drawing for engineers. Previous research in automated PIC routing largely relies on off-the-shelf algorithms designed for electrical circuits, which only support high-level route planning to minimize waveguide crossings. It is not customized to handle unique photonics-specific routing constraints and metrics, such as curvy waveguides, bending, port alignment, and insertion loss. These approaches struggle with large-scale PICs and cannot produce real layout geometries without design-rule violations (DRVs). This highlights the pressing need for electronic-photonic design automation (EPDA) tools that can streamline the physical design of modern PICs. In this paper, for the first time, we propose an open-source automated PIC detailed routing tool, dubbed APR, to generate DRV-free PIC layout for large-scale real-world PICs. APR features a grid-based curvy-aware A* engine with adaptive crossing insertion, congestion-aware net ordering and objective, and crossing-waveguide optimization scheme, all tailored to the unique property of PIC. On large-scale real-world photonic computing cores and interconnects, APR generates a DRV-free layout with 14% lower insertion loss and 6.25x speedup than prior methods, paving the way for future advancements in the EPDA toolchain. Our codes are open-sourced at https://github.com/ScopeX-ASU/APR.

==> texlib/ieee_normal.tex <==


\usepackage{algpseudocode}                                 %
\usepackage{algorithm}
\usepackage{graphicx}                                      %
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage[subrefformat=parens,farskip=0pt,justification=centering]{subfig}
\usepackage{color}
\usepackage{cite}                                          %
\usepackage{comment}                                       %
\usepackage{soul}                                          %
\soulregister\cite7
\soulregister\ref7
\soulregister\pageref7
\usepackage{amsthm}
\usepackage{etoolbox}                                      %
\usepackage{url}
\usepackage{nth}                                           %
\usepackage{bm}                                            %
\usepackage{courier}
\usepackage{balance}
\usepackage{threeparttable}
\usepackage[bookmarks=false]{hyperref}                     %
\hypersetup{
    colorlinks = true,
    citecolor  = blue,
    linkcolor  = blue,
    urlcolor   = blue,
}
\usepackage{filecontents}                                  %
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=newest}
\usepackage{caption} 
\captionsetup[table]{skip=4pt}
\setlength{\columnsep}{16pt}                               %
\definecolor{CUHKorange}{RGB}{244,106,18} %
\definecolor{CUHKblue}{RGB}{0,111,190}    %
\definecolor{CUHKgreen}{RGB}{0,127,128}   %
\definecolor{CUHKred}{RGB}{228,46,36}     %
\definecolor{CUHKyellow}{RGB}{198,148,34} %
\definecolor{CUHKdark}{RGB}{114,44,114}   %
\definecolor{CUHKmiddle}{RGB}{144,44,144} %
\definecolor{CUHKlight}{RGB}{167,44,167} 

\newtheorem{myproblem}{\textbf{Problem}}
\newtheorem{mydefinition}{\textbf{Definition}}
\newtheorem{mytheorem}{\textbf{Theorem}}
\newtheorem{mycorollary}{\textbf{Corollary}}
\newtheorem{mylemma}{\textbf{Lemma}}
\newtheorem{myclaim}{\textbf{Claim}}
\newtheorem{myapplication}{\textbf{Application}}
\newtheorem{myconjecture}{Conjecture}
\newtheorem{myprop}{Property}

\algrenewcommand\textproc{\texttt}
\newcommand{\tabincell}[2]{
    \begin{tabular}{@{}#1@{}}#2\end{tabular}
}

\makeatletter
\let\OldStatex\Statex
\renewcommand{\Statex}[1][3]{%
  \setlength\@tempdima{\algorithmicindent}%
  \OldStatex\hskip\dimexpr#1\@tempdima\relax
}
\makeatother


\RequirePackage[normalem]{ulem} %
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %
\providecommand{\DIFadd}[1]{{\protect\color{blue}{#1}}}                           %
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}                       %
\providecommand{\DIFaddbegin}{}                                                   %
\providecommand{\DIFaddend}{}                                                     %
\providecommand{\DIFdelbegin}{}                                                   %
\providecommand{\DIFdelend}{}                                                     %
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}}                                        %
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}}                                        %
\providecommand{\DIFaddbeginFL}{}                                                 %
\providecommand{\DIFaddendFL}{}                                                   %
\providecommand{\DIFdelbeginFL}{}                                                 %
\providecommand{\DIFdelendFL}{}                                                   %




